Joint Time-and Event-Triggered Scheduling in the Linux Kernel

There is increasing interest in using Linux in the real-time domain due to the emergence of cloud and edge computing, the need to decrease costs, and the growing number of complex functional and non-functional requirements of real-time applications. Linux presents a valuable opportunity as it has rich hardware support, an open-source development model, a well-established programming environment, and avoids vendor lock-in. Although Linux was initially developed as a general-purpose operating system, some real-time capabilities have been added to the kernel over many years to increase its predictability and reduce its scheduling latency. Unfortunately, Linux currently has no support for time-triggered (TT) scheduling, which is widely used in the safety-critical domain for its determinism, low run-time scheduling latency, and strong isolation properties. We present an enhancement of the Linux scheduler as a new low-overhead TT scheduling class to support offline table-driven scheduling of tasks on multicore Linux nodes. Inspired by the Slot shifting algorithm, we complement the new scheduling class with a low overhead slot shifting manager running on a non-time-triggered core to provide guaranteed execution time to real-time aperiodic tasks by using the slack of the time-triggered tasks and avoiding high-overhead table regeneration for adding new periodic tasks. Furthermore, we evaluate our implementation on server-grade hardware with Intel Xeon Scalable Processor.

==> LRS.tex <==
% !TEX root = ../paper.tex
\svnid{$Id$}\vspace{-0.1cm}
\section{Time-Triggered Resource Scheduling}\label{sec:TT}
This section describes our CPU-and memory bandwidth-aware offline scheduler that generates a \gls{TT} scheduling table for use with an LRM. 
%The LRM stores this offline generated scheduling table and controls a simple low overhead runtime dispatcher on its node that dispatches \glspl{VM} as per the table. 
For simplicity of explanation, we assume each \gls{VM} requires only one virtual CPU.
We consider \gls{SC} \glspl{VM} with a constant amount of memory accesses. Each \gls{VM} is granted at most one memory access at a time, resulting in waiting times for accesses from other \glspl{VM}. 
We assume that ongoing memory access is not preemptible. 

We consider global time whose progress is triggered by equidistant events, $\epsilon_0, \epsilon_1,\ldots, \epsilon_\infty$ \cite{schorr}. We consider a sparse time base where the time duration separating two of these events, $\epsilon_s$ and $\epsilon_{s+1}$ respectively, is called a \textit{Slot}, $S_s$. $\Delta t_{S}$ is the duration of each slot.
Slot $start(S_0)=\epsilon_0$, $end(S_1)=start(S_2)=\epsilon_1$ and so on. 
A multicore slot on a cloud node can run $P$ \glspl{VM} at a time, where $P$ is the total number of CPU cores. The sum of the reserved bandwidth for each of the \glspl{VM} running in a single slot must not exceed the maximum allowed bandwidth of the node ($BW_{max}$).
A slot S($\Delta t_{S}$, $BW^p$, M, SBW) is described by Table \ref{tab:summary_slot}. %Based on the global slot-shifting algorithm \cite{schorr}, we set $\Delta t_{S}$ interval to $10 ms$.

\begin{table}[b]
	\centering\vspace{-0.5cm}
	\begin{tabular}{|p{4.5cm}|p{3.5cm}|}
		\hline
		A slot is described by: & Units \\
		\hline
		CPU Allocation $\Delta t_{S}$ & in time units, e.g., milliseconds \\
		\hline
		Memory Bandwidth allocation $BW^p$ & in memory accesses per regulation interval of a slot \\
		\hline
		Mapping $M$ of \gls{VM}(s) to CPU cores & M:$\tau \rightarrow p$\\
		\hline
		Spare (unused) Memory Bandwidth $SBW$ & in memory accesses per regulation interval of a slot \\
		\hline
	\end{tabular}
	\caption{Summary of Slot}\vspace{-0.1cm}
	\label{tab:summary_slot}
\end{table}

We define a \textit{Regulation interval} as a slot-wide parameter that is small to enforce $BW^p$ effectively. In the most straightforward implementation, the Regulation interval can be equal to the slot length. However, this would lead to very coarse memory bandwidth regulation. Although a small regulation interval is better for predictability, there is a practical limit on reducing the period due to interrupt and scheduling overhead; based on MemGuard \cite{memguard}, we set the regulation interval to $1 ms$.

We define a \gls{VM} $\tau$ with a tuple $\langle r,C^s,d,\phi, C^m \rangle$, where $r$ is the start slot of the \gls{VM}, $C^s$ is worst-case execution time of the \gls{VM} (in slots) when running in isolation and with no memory bandwidth restrictions, $d$ is the absolute deadline of the \gls{VM} (in slots), $\phi$ is the maximum number of memory accesses the \gls{VM} is allowed to issue per regulation interval, and $C^m$ is the worst-case execution time of the \gls{VM} (in slots) when restricting the memory bandwidth of the \gls{VM} to $\phi$ accesses per regulation interval. 
Note that $C^m$ is dependent on $\phi$; thus, the memory bandwidth of the task will increase as $\phi$ increases, causing $C^m$ to decrease. 
In other words, each value for $\phi$ will produce a different $C^m$ for each \gls{VM}. 
Moreover, \cite{nowotsch2014multi} demonstrated that the latency for a single memory access operation increase significantly when the number of active cores increases.   

We created a heuristic algorithm to assign slots to \glspl{VM} before runtime, considering the points mentioned earlier. $\phi$ and its corresponding $C^m$ are determined in such a way that the \glspl{VM} are schedulable while using the minimum possible bandwidth from $BW_{max}$ on the node. The result of the heuristic is a cyclic scheduling table with slots consisting of $BW^p_s$ values, $M_s$, and $SBW_s$ per slot $s$. 

This scheduling table is stored by the LRM of a cloud node (Figure \ref{fig:local}). The LRM runs on a node's non-TT (housekeeping) core and executes before the start of each slot (only on this core). 
The LRM controls a simple low overhead runtime dispatcher on its node and dispatches \glspl{VM} as per the mapping $M_s$ in the scheduling table. At the start of a slot, a \gls{TT} dispatcher stops \glspl{VM} currently executing and dispatches the new \glspl{VM}. The LRM also controls a scheduler similar to Memguard \cite{memguard} which reserves memory bandwidth $BW^p_s$ for core $p$ during slot $s$. 
If a \gls{VM} finishes execution early, the $M_s$ is updated accordingly in future slots, and the $BW^p_s$ value stored for that \gls{VM} in future slots is freed (as a result, $SBW$ increases for those slots).
Moreover, at end of a slot, each LRM updates any change in $SBW$, $M$ and status of applications to the GRM.
\begin{figure}[htb]
	\centering\vspace{-0.3cm}
	\includegraphics[width=\columnwidth]{standalone_figures/ttlrs.png}\vspace{-0.125cm}
	\caption{Local Resource Manager (LRM) and TT Dispatcher}\vspace{-0.5cm}
	\label{fig:local}
\end{figure}

\section{Adding Flexibility to TT Scheduling}\label{sec:ET}
To add new \glspl{VM} to the scheduling table at runtime, we execute an algorithm inspired by Slot-Shifting \cite{schorr} in the LRMs. This section gives a high-level overview of this algorithm.

We group a set of consecutive slots into a \textit{capacity interval} (or simply \textit{interval} for short). We define an interval as a set of consecutive slots that possess the same mapping $M$ of \gls{VM}(s) to CPU cores. In other words, a new interval starts on slot $S_s$ when the set of \glspl{VM} assigned to this slot are different from the ones assigned to the previous slot ($S_{s-1}$). 
Intervals may contain some cores that haven't been assigned any \gls{VM}, resulting in idle slots within the interval. These slots define the \textit{Spare CPU Capacity} of an interval $\iota_f$ ($SCPU_f$), which can be used to schedule \gls{ET} \glspl{VM}. Furthermore, each core $C_n$ is reserved memory bandwidth $BW_f^n$ depending on which \gls{VM} 
%is assigned to it for interval $\iota_f$. 
it was assigned for interval $\iota_f$. 
The unreserved memory bandwidth for $\iota_f$ is denoted as $SBW_f$. 

The LRM executes an \textit{acceptance test} and a \textit{guarantee routine} to handle new \gls{ET} \gls{SC} \gls{VM}(s) (as in  Slot-Shifting \cite{schorr}). 
When a new \gls{VM} arrives, the acceptance test determines if there is enough available $SCPU$ and $SBW$ in the intervals before the \gls{VM}'s deadline. If the test is successful, the guarantee routine is executed to add the \gls{VM} to the scheduling table and update the $SCPU$ and $SBW$ of all affected intervals. As a result, this routine guarantees the resource allocation to the new accepted VM.
Note that, unlike previous work, our acceptance test and guarantee routine take into account the node's $SBW$ and the \gls{VM}'s $\phi$.% of the \gls{VM}.

At run-time, The LRM executes any \gls{VM} assigned to the current interval (via the dispatcher). In idle slots, it executes any \gls{SC} \glspl{VM} that are available but not assigned to the interval. If no \gls{SC} \glspl{VM} are available, the LRM selects non-critical \glspl{VM}. 

If an LRM is unable to accept a new \gls{SC} \gls{VM} due to unavailability of resources, the LRM requests the GRM for cloud-wide adaptation. The GRM, in turn, searches for another node with more appropriate resource availability and dispatches the \gls{VM} to that node.
Similarly, if a node is unable to execute an existing \gls{VM} or the VM does not achieve the desired \gls{QoS} due to a change in availability of resources, the resource management layer redeploys the VM to another node in the cloud. The change in availability of the resources can result from resource failure or a change in resource demand.




%Additionally, each \gls{VM} is assigned a budget for their designated intervals; this budget is updated at run-time when the \gls{VM} is selected to run. \gls{VM}'s are allowed to migrate between cores, so the assigned core for a \gls{VM} may vary from one interval to the next. The second part of the guarantee algorithm consists in reducing the spare capacity of the corresponding core in each interval by the number of slots the \gls{VM} has been assigned within that interval. Additionally, we must reduce the spare bandwidth of the intervals where any extra bandwidth was used for the core where this new \gls{VM} was assigned. In case of \gls{BE} \gls{VM}(s), no acceptance test nor guarantee algorithm is needed because they only execute in idle slots weren't being used for other \gls{SC}. %\gls{VM}(s) anyway. Futheremore, no guarantee is made with respect to the memory bandwidth these \gls{VM}(s) are reserved. 

%At run-time, any \gls{VM} assigned to a core for the current interval is selected to execute and their budget is reduced by $1$. If a core is idle for the current slot then any \gls{SC} \gls{VM} is chosen to execute. If the \gls{VM} is allowed to run with it's necessary bandwidth, then the budget of it's first interval it is assigned to is decreased by one and the spare capacity of this core is increased by one. If the \gls{VM} is not allowed to run with it's necessary bandwidth then no modification is made to it's first interval. Note that when the budget for the interval reaches $0$, the \gls{VM} is deassigned from the interval. If no \gls{SC} \gls{VM}'s are available then any non-critical/\gls{BE} \gls{VM}(s) are selected to run. Whenever a \gls{VM} executes for a slot it was not assigned, the spare capacity for the core is reduced by $1$; the same applies when a core is idle for the current slot. 

%In the case a node is unable to accept a new \gls{SC} \gls{VM}, the resource management layer searches for another node with more appropriate resource availability and dispatches the \gls{VM} to that node.
%If a node is unable to execute one or more non-critical/\gls{BE} \gls{VM} due to limited availability of resources, the resource management layer dispatches the \gls{VM}(s) to other nodes with more resource availability. The resource management layer also dispatches the non-critical/\gls{BE} \gls{VM} to other nodes with more resource availability if they do not acheive the targeted \gls{QoS} on the current node.



%%%%% OLD VERSION
%We group consecutive slots that possess the same mapping M of \gls{VM}(s) to CPU cores into a \textit{capacity interval} $\iota$ (or simply \textit{interval} for short). 
%The start of interval 0 ($\iota_0$) is equal to the start of Slot 0 which has a mapping $M_0$. In our case, $start(\iota_0)=start(S_0)=\epsilon_0=0$. The interval $\iota_0$ ends at the end of slot $S_s$ where $M_s\neq M_{s+1}$. A new interval $\iota_1$ starts at the start of the next slot, $start(S_{s+1})$. The last interval ends at $S_S$, where $S$ is the total number of slots. To summarize, intervals are created using the following criteria:

%\begin{itemize}
%	\item Start of First interval $start(\iota_0) = start(S_0) (=0)$
%	\item End of Last interval  $end(\iota_L) = end(S_S)$
%	\item For all intervals $\iota_i$, 
%	\begin{equation*}
%		start(\iota_i) = start(S_{s+1})|M_s\neq M_{s+1}
%	\end{equation*}
%	\begin{equation*}
%		end(\iota_i) = end(S_s)|M_s\neq M_{s+1}
%	\end{equation*}
%	Note: $start(S_{s+1})=end(S_{s})$
%\end{itemize}
%
%The length of an interval is defined as: 
%
%\begin{equation}\label{eq:int_length}
%	|\iota_i| = end(\iota_i)-start(\iota_i)
%\end{equation}

%Given that our mapping $M$ is constant throughout an interval $\iota_f$, any \gls{VM} $\tau_j$ assigned to $\iota_f$ will be mapped to one specific core $C_k$ s.t. $k\in\{0,P\}$ for the duration of the interval. Similarly, another \gls{VM} $\tau_l$ also assigned to $\iota_f$, will be assigned to a core $C_m$, where $m \neq k$. A core $C_n$ that isn't assigned a \gls{VM} will contain idle slots. The number of idle slots for $C_n$ within an interval is known as \textit{spare CPU Capacity} of $C_n$ for $\iota_f$ ($SC_f^n$). According to this definition, a core may have a maximum spare CPU capacity equal to the length of the interval and a minimum spare CPU capacity of $0$.

%Each core $C_n$ is reserved a certain percentage of memory bandwidth $BW_f^n$ depending on which task is assigned to it for interval $\iota_f$. The remaining percentage of memory bandwidth in the interval is known as \textit{spare Memory Bandwidth} of interval $\iota_f$ ($SBW_f$). 

%Similar to Slot-shifting \cite{fohler}, an \textit{acceptance test} is executed for new \gls{ET} \gls{SC} \gls{VM}(s) at run-time. The acceptance test determines if there is enough available spare capacity before the \gls{VM}'s deadline and that it will receive the necessary memory bandwidth within these available slots. Once accepted, the \textit{gaurantee algorithm} \cite{fohler, schorr} is executed; this adds the \gls{VM} to the scheduling table along with a list of the intervals and cores it is assigned to. Additionally, each \gls{VM} is assigned a budget for their designated intervals; this budget is updated at run-time when the \gls{VM} is selected to run. \gls{VM}'s are allowed to migrate between cores, so the assigned core for a \gls{VM} may vary from one interval to the next. The second part of the guarantee algorithm consists in reducing the spare capacity of the corresponding core in each interval by the number of slots the \gls{VM} has been assigned within that interval. Additionally, we must reduce the spare bandwidth of the intervals where any extra bandwidth was used for the core where this new \gls{VM} was assigned. In case of \gls{BE} \gls{VM}(s), no acceptance test nor guarantee algorithm is needed because they only execute in idle slots weren't being used for other \gls{SC}. %\gls{VM}(s) anyway. Futheremore, no guarantee is made with respect to the memory bandwidth these \gls{VM}(s) are reserved. 
%
%At run-time, any \gls{VM} assigned to a core for the current interval is selected to execute and their budget is reduced by $1$. If a core is idle for the current slot then any \gls{SC} \gls{VM} is chosen to execute. If the \gls{VM} is allowed to run with it's necessary bandwidth, then the budget of it's first interval it is assigned to is decreased by one and the spare capacity of this core is increased by one. If the \gls{VM} is not allowed to run with it's necessary bandwidth then no modification is made to it's first interval. Note that when the budget for the interval reaches $0$, the \gls{VM} is deassigned from the interval. If no \gls{SC} \gls{VM}'s are available then any non-critical/\gls{BE} \gls{VM}(s) are selected to run. Whenever a \gls{VM} executes for a slot it was not assigned, the spare capacity for the core is reduced by $1$; the same applies when a core is idle for the current slot. 
%
%In the case a node is unable to accept a new \gls{SC} \gls{VM}, the resource management layer searches for another node with more appropriate resource availability and dispatches the \gls{VM} to that node.
%If a node is unable to execute one or more non-critical/\gls{BE} \gls{VM} due to limited availability of resources, the resource management layer dispatches the \gls{VM}(s) to other nodes with more resource availability. The resource management layer also dispatches the non-critical/\gls{BE} \gls{VM} to other nodes with more resource availability if they do not acheive the targeted \gls{QoS} on the current node.


%%%%% OLD VERSION

% First any \gls{SC} \gls{VM} assigned to the core in the current interval is selected; if none are assigned, i.e., if the we are in an idle slot for this core, any other \gls{SC} \gls{VM} is assigned.  if a task is assigned to a core for the current slot in interval, this task is executed. If the core will be idle for the slot, then a \gls{SC} \gls{VM} is assigned to the core. If the \gls{VM} is reserved it's necessary bandwidth for this slot, then the spare capacity of the first interval this \gls{SC} \gls{VM} is assigned to must be increased by one. No modifications are made to the spare capacity if this is not the case because the \gls{VM} will execute with limited memory bandwidth. If no other \gls{SC} \gls{VM} are available then any \gls{BE} \gls{VM} is chosen to execute for that slot. 
% talk about runtime execution maybe. 
%, only the spare capacity for the current interval is reduced (which was going to be reduced anyway because it was an idle slot).



==> Makefile <==
paper=paper.pdf
main=paper.tex

srcs=
figtex=standalone_figures/ 
figpdf=$(patsubst %.tex,%.pdf,$(figtex))
bibs=references.bib
figpdf=$(addsuffix .pdf, $(basename $(wildcard standalone_figures/*.tex)))

all: $(paper)

figures: $(figpdf)

standalone_figures/%.pdf:  standalone_figures/%.tex
	@mkdir -p standalone_figures/tmp && echo "Successfully created standalone_figures/tmp folder"
	@printf "Creating $@ ... \n"
	@(pdflatex -output-directory=standalone_figures/tmp -halt-on-error $<)2> standalone_figures/tmp/pdf.log \
                1> standalone_figures/tmp/pdf.out || \
                ( printf "... FAILED!!!! (check standalone_figures/tmp/" && \
                        printf "$(patsubst %.tex,%.log,$<) " && \
                        printf "for errors, " && \
                        printf "specially the lasts lines)\n" && exit 1 )
	@cp standalone_figures/tmp/*.pdf standalone_figures/
	@printf "...done\n"

tmp/paper.bbl:
	@bibtex paper

$(paper): $(main) $(srcs) $(bibs) $(figpdf)
	@echo "removing paper.pdf"
	@rm -rf paper.pdf
	@echo "required figure pdfs in standalone_figures directory:" $(figpdf)
	@mkdir -p tmp && echo "Successfully created tmp folder"
	@printf "Creating $@ ...\n"
	@(latexmk -bibtex -shell-escape -pdf -quiet -output-directory=tmp -pdflatex='pdflatex -synctex=1' -use-make $<) \
		2> tmp/latexmk.log \
		1> tmp/latexmk.out || \
		( printf "... FAILED!!!! (check tmp/" && \
			printf "$(patsubst %.tex,%.log,$<) " && \
			printf "for errors, " && \
			printf "specially the lasts lines)\n" && exit 1 )
	@printf "...done. Make once more incase you have done changes to the glossary entries\n"
	@cp tmp/paper.synctex.gz .
	@cp tmp/paper.pdf .

clean:
	rm -rf paper.pdf
distclean:
	rm -rf tmp
	rm -rf paper.pdf
	rm -rf standalone_figures/*.pdf
	rm -rf standalone_figures/tmp


==> resourcemanagement.tex <==
% !TEX root = ../paper.tex
\svnid{$Id$}
\section{Resource Management Layer for Cloud}
%\ggcomment{2 column}
A hypervisor 
alone is not adequate to meet all the requirements for \gls{SC} \glspl{VM} due to contention in shared resources of cloud nodes \cite{gala:railway}.
%Safety-critical systems require careful planning and allocation of these resources.
Most cloud hypervisors only support partitioning or allocation of few selected node resources among the \glspl{VM}; for example, allocating CPU time or memory space to \glspl{VM}.
They require additional mechanisms for the allocation of other shared resources.
Moreover, they only consider a single node at a time.
If the applications, resource availability, or cloud configurations change, obtaining assumptions about cloud resources becomes complicated and requires cloud-wide coordinated decision-making and resource management: {\em resource management layer}.

Our resource management layer complements the cloud hypervisors to support the allocation of additional shared resources.
It enables the cloud to make resource management decisions to leverage the availability of resources in all the nodes; this helps to meet end-to-end constraints, 
%It enables the cloud to leverage the availability of resources in all nodes to make resource management decisions that help to meet end-to-end constraints, 
provide fault-tolerance,
or increase cloud-wide efficiency.
The resource management layer is inspired by the DREAMS project resource management \cite{DREAMS}. 
Unlike the offline (static) assignment of resources to \glspl{VM} in DREAMS, 
our resource management layer adds flexibility to enable dynamic resource assignment in the cloud.
The SECREDAS project's safety-critical railway use case \cite{gala:railway} indicated the requirement of a similar resource management layer in a private cloud.

The main idea of the resource management layer is based on decoupling the node-level scheduling from the cloud-wide resource management.
It consists of node-level local resource managers (LRMs) and a cloud-level Global resource manager (GRM). 
The LRMs run on top of the hypervisor on each node. They complement the hypervisor to ensure the partitioning and allocation of resources not taken care of by the hypervisor (memory bandwidth in our case).
They support \gls{TT} triggered scheduling (Section III) and provide flexibility to add ET \glspl{VM} at runtime without the need of high-overhead table regeneration (Section IV).
In addition, the LRMs monitor the availability, demand, and health of resources as well as the applications for QoS and behavior (such as a potential deadline miss \cite{DREAMS}).
Based on the monitoring information, the LRMs make node-level resource scheduling decisions and keep the GRM updated about the status of a node.

The GRM controls and coordinates LRMs of all nodes. It supports reconfiguration of the cloud upon changes in the availability of resources and demands of applications at runtime. It makes reconfiguration decisions by maintaining a cloud-wide view of resources and applications based on monitoring updates from the LRMs.
Any cloud-wide decisions made by the GRM are sent to the LRMs involved in the decision. These LRMs enforce the decision on their nodes via node-level scheduling. Existing approaches implement the GRM on a single node \cite{DREAMS} or distributed across several nodes for fault-tolerance \cite{blockchainWIP}. This paper focuses on how LRMs can provide memory bandwidth-aware \gls{TT} scheduling (Section \ref{sec:TT}) and flexibility to add \gls{ET} \glspl{VM} at runtime (Section \ref{sec:ET}).

%Figure \ref{fig:rt-cloud} shows the resource management layer in the envisaged RT-cloud. 
%\begin{figure}[t] 
%	\centering
%	%\def\svgwidth{\columnwidth}
%	%    \input{figures/rt-cloud.tex}
%	\includegraphics[width=\columnwidth]{figures/rt-cloud.png}
%	\caption{Envisaged RT-Cloud}
%	\label{fig:rt-cloud}
%\end{figure}
%
%The resource management layer is realized by using node-level \glspl{lrm} to monitor and orchestrate node resources individually, 
%and disseminate the state of resources to a \gls{grm} (Figure \ref{fig:arch}). 
%The \glspl{lrm} on each cloud node consists of the following:
%\begin{figure}[h]
%	\centerline{\includegraphics[width=\linewidth]{standalone_figures/rm}}
%	\caption{Resource Management Layer Components}
%	\label{fig:arch}
%\end{figure}
%\paragraph{Monitors (MONs)} Multiple monitors are used by the \gls{lrm} to monitor the resources for utilization, availability, health, \etc, 
%and applications (and hypervisor) for run-time behavior.
%Some examples are CPU core utilization or memory bandwidth monitors.
%\paragraph{Local Resource Schedulers (LRSs)} Multiple schedulers on Node are used by the \gls{lrm} for resource reservation/scheduling
%and controlling access of applications to resources.
%Some examples are 
%\gls{TT} scheduler,
%and memory-bandwidth enforcing techniques.
%
%A single (central) \gls{grm} \cite{DREAMS} or a distributed \gls{grm} \cite{blockchainWIP}  participates in global resource management to enable cloud-wide adaptability and deals with on situations like resource failures, overloads, \etc 
%The \gls{lrm} of each node sends periodic updates (based on information from the \glspl{mon}) to the \gls{grm} based on the monitoring information.
%These resource updates are used by the \gls{grm} to maintain a cloud-wide view of resources and make global resource re-orchestration decisions. 
%Any global decisions made by the \gls{grm} are sent to the \glspl{lrm} of the nodes involved in the re-orchestration.
%The \glspl{lrm} enforce the global re-orchestration decision of the \gls{grm} via the respective \glspl{lrs}.

